Applying consensus and replication securely with FLAQR

Availability is crucial to the security of distributed systems, but guaranteeing availability is hard, especially when participants in the system may act maliciously. Quorum replication protocols provide both integrity and availability: data and computation is replicated at multiple independent hosts, and a quorum of these hosts must agree on the output of all operations applied to the data. Unfortunately, these protocols have high overhead and can be difficult to calibrate for a specific application's needs. Ideally, developers could use high-level abstractions for consensus and replication to write fault-tolerant code by that is secure by construction. This paper presents Flow-Limited Authorization for Quorum Replication (FLAQR), a core calculus for building distributed applications with heterogeneous quorum replication protocols while enforcing end-to-end information security. Our type system ensures that well-typed FLAQR programs cannot_fail_ (experience an unrecoverable error) in ways that violate their type-level specifications. We present noninterference theorems that characterize FLAQR's confidentiality, integrity, and availability in the presence of consensus, replication, and failures, as well as a liveness theorem for the class of majority quorum protocols under a bounded number of faults.

==> paperversions.tex <==
% Sets options for different versions of a peer-reviewed paper. Cannot
% be a LaTeX package because it must often be used _before_
% \documentclass. Use as follows:
%
%   \def\paperversion{draft}
%   \def\anonymoussubmission{0} % optional. Value should be 0 or 1 if defined.
%   \input{paperversions}
%
% In addition to 'draft', the following document versions are
% supported: markup, local, submission, final, finaldraft, web, tr, trdraft
%
% markup: internal draft for paper markup. Does not use submission formatting or show comments.
% draft: internal draft with standard layout (comments shown, blinded if necessary)
% local: version for local review (not blinded, warning re distribution)
% submission: submission for review (blinded if necessary)
% final: camera-ready (not blinded, no distribution warning)
% finaldraft: like final, but comments shown
% web: version to post on a website. Like final, but with page
%      numbers and possibly information about where paper was published.
% tr: technical report
% trdraft: technical report with comments shown
%
% The following \if conditions are defined appropriately depending on
% which version is chosen:
%
\newif\ifsinglecolumn\singlecolumnfalse
\newif\ifwidemargins\widemarginsfalse
\newif\ifwarning\warningfalse
\newif\ifshowcomments\showcommentsfalse
\newif\ifblinded\blindedfalse
\newif\ifreport\reportfalse
\newif\ifcopyrightspace\copyrightspacefalse
\newif\ifacknowledgments\acknowledgmentsfalse
\newif\ifshowpagenumbers\showpagenumberstrue
\newif\iffinalformat\finalformatfalse
\newif\ifweb\webfalse

% The condition \ifblinded is turned on if the file
% .blinded exists or if \anonymoussubmission is defined to be 1, unless
% overridden by the document version chosen. The local, final, tr,
% trdraft, and web versions are not blinded.
%
\ifx\anonymoussubmission\undefined
  \typeout{** Assuming venue has non-anonymous submission}
\else
  \if\anonymoussubmission 1
    \blindedtrue
  \else
    \blindedfalse
  \fi
\fi
\IfFileExists{.blinded}{\blindedtrue}

\def\xxmarkup{0}
\def\xxdraft{1}
\def\xxlocal{2}
\def\xxsubmission{3}
\def\xxfinal{4}
\def\xxtr{5}
\def\xxtrdraft{6}
\def\xxfinaldraft{7}
\def\xxweb{8}
\def\xxblindtr{9}

\ifx\paperversion\xxxxundefined
\PackageError{paperversions}{*** No valid document version was specified.
Macro paperversions must be be defined as one of (markup, draft,
local, submission, final, web, tr, trdraft)}
\fi

\def\xxversion{\csname xx\paperversion\endcsname}
\newif\ifsawversion\sawversionfalse

\ifcase\xxversion\relax
%markup
    \widemarginstrue
    \singlecolumntrue
    \warningtrue
    \sawversiontrue
\or %draft
    \warningtrue
    %\showcommentstrue
    \sawversiontrue
\or %local
    \warningtrue
    \showcommentsfalse
    \blindedfalse
    \sawversiontrue
    \acknowledgmentstrue
\or %submission
    \sawversiontrue
\or %final
    \blindedfalse
    \sawversiontrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \showpagenumbersfalse
    \finalformattrue
\or %tr
    \singlecolumntrue
    \blindedfalse
    \sawversiontrue
    \reporttrue
    \acknowledgmentstrue
    \webtrue
\or %trdraft
    \blindedfalse
    \singlecolumntrue
    \showcommentstrue
    \sawversiontrue
    \reporttrue
\or %finaldraft
    \blindedfalse
    \showcommentstrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \sawversiontrue
    \finalformattrue
\or %web
    \blindedfalse
    \sawversiontrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \finalformattrue
    \webtrue
\or %blindtr
    \singlecolumntrue
    \blindedtrue
    \acknowledgmentsfalse
    \sawversiontrue
    \reporttrue
    \webtrue
\fi

\ifsawversion
\else
    \typeout{*** Internal error: no valid document version processed! ***}
\fi

% Cleanup.
\let\xxmarkup=\undefined
\let\xxlocal=\undefined
\let\xxsubmission=\undefined
\let\xxfinal=\undefined
\let\xxfinaldraft=\undefined
\let\xxtr=\undefined
\let\xxtrdraft=\undefined
\let\xxweb=\undefined
\let\xxblindtr=\undefined
\let\xxversion=\undefined

